A Case for Fine-grain Coherence Specialization in Heterogeneous Systems

Hardware specialization is becoming a key enabler of energyefficient performance. Future systems will be increasingly heterogeneous, integrating multiple specialized and programmable accelerators, each with different memory demands. Traditionally, communication between accelerators has been inefficient, typically orchestrated through explicit DMA transfers between different address spaces. More recently, industry has proposed unified coherent memory which enables implicit data movement and more data reuse, but often these interfaces limit the coherence flexibility available to heterogeneous systems. This paper demonstrates the benefits of fine-grained coherence specialization for heterogeneous systems. We propose an architecture that enables low-complexity independent specialization of each individual coherence request in heterogeneous workloads by building upon a simple and flexible baseline coherence interface, Spandex. We then describe how to optimize individual memory requests to improve cache reuse and performance-critical memory latency in emerging heterogeneous workloads. Collectively, our techniques enable significant gains, reducing execution time by up to 61% or network traffic by up to 99% while adding minimal complexity to the Spandex protocol.

==> mem_opt_thesis.tex <==
\chapter{Dynamic Coherence Specialization}
\label{chap:mem-opt}

%\section{Background}
%\label{sec:mem-opt-background}

%In this section I propose three sets of extensions which exploit some of the most common information available from heterogeneous programming models and describe how they can be used to improve hardware efficiency.
%Coherence locality hints exploit information about access locality, commonly available in programming models which use hierarchical communication or partitioned global address spaces~\cite{HowesMunshi2015,YelickBonachea2007}. Coherent queues exploit information about dataflow between different tasks, which is available in many dataflow programming languages~\cite{ZahariaChowdhury2010,AbadiAgarwal2016}. Coherent DMA exploits information about access granularity, and relies on the DMA primitive commonly used by specialized systems which access data in bulk.
%All three adhere to the common SC-for-DRF memory model.
%Completing all three of these extensions will not be possible in the coming months, but with your feedback I hope to select and refine one or two of these proposals to develop for my final defense.
%-emerging programming interfaces contain locality, dataflow, memory demand info.
%
%-spandex can exploit this information naturally
%
%-spandex can be extended further to take advantage of this
The flexibility of Spandex offers new opportunities for memory system performance optimization.
Although Chapter~\ref{chap:spandex} focuses primarily on Spandex's ability to interface a wide variety of coherence protocols that use fixed request types for each access, there is no need to restrict devices in this way.
A local cache in a Spandex system may dynamically choose request types based on the properties of the workload being executed.
%In addition to offering dynamic request specialization to heterogeneous workloads with varying memory demands, 
Spandex requests can also be extended with additional optimizations designed to improve performance for specific access patterns.
%For example, the protocol at the Spandex LLC may be extended to optionally forward write-through requests to the current owner without revoking ownership, in a similar way to how self-invalidating reads are handled. 
%This can be beneficial when the latency on the consumer side of some inter-device communication affects performance more than the latency of the producer.
Unlike MESI-based heterogeneous protocols, which suffer from high complexity and a multitude of blocking states, 
Spandex is able to implement extensions with minimal effort or added complexity.

%When combined with a flexible memory system like Spandex, this information can be exploited to match memory system specialization to the specific memory demands of a workload.
%Although Chapter~\ref{chap:spandex} focuses primarily on Spandex's ability to interface a wide variety of coherence protocols which use fixed request types for each access, there is no need to restrict devices in this way.
%A local cache in a Spandex system may dynamically choose request types based on the properties of the workload being executed.

%In addition to offering dynamic request specialization to heterogeneous workloads with varying memory demands, Spandex can be easily extended with further optimizations.
%For example, the protocol at the Spandex LLC may be extended to optionally forward write-through requests to the current owner without revoking ownership, in a similar way to how self-invalidating reads are handled. 
%This can be beneficial when the latency of the read in some remote communication affects performance more than the latency of the write.
%Unlike MESI-based heterogeneous protocols, which suffer from high complexity and a multitude of blocking states, 
%Spandex is able to implement such extensions with minimal effort or added complexity.
% if time: direct forwarding

%We refer to the above optimiziations as memory performance extensions. 
Importantly, while this interface flexibility allows a device to choose between multiple types of loads and stores, it does not add complexity to the DRF memory model.
No matter which request type is used for a load, store, or atomic access, the functional semantics of that access do not change.

In the following sections we describe a set of specialized Spandex request types, we evaluate the benefits of dynamic request selection effects on a set of applications, and we offer a simple complexity comparison with a more conventional heterogeneous protocol.

\section{Specialized Coherence Overview}
\label{sec:mem-opt-design}

The Spandex protocol offers dynamic flexibility in three dimensions (summarized in table~\ref{table:coherence_strategies}): 
stale data invalidation, write propagation, and granularity.
Dynamic selection of request types in these dimensions requires no change to the Spandex protocol.
We also consider two optimizations that require modification to baseline Spandex: write-through request forwarding and owner prediction.

\textbf{Dynamic stale data invalidation}: Load accesses can generate writer-invalidated reads (ReqS) if reuse across synchronization boundaries is expected.
Since requesting Shared state will prevent requested data from being self-invalidated at synchronization points, this can improve cache efficiency, reducing execution time and network traffic.
If reuse across synchronization points is not expected to be high and/or memory throughput is judged to be more important to performance,
a load access may generate a self-invalidating read instead and avoid the latency and network overheads of writer-initiated invalidation.

\textbf{Dynamic write propagation}: Stores and atomic operations can use ownership requests (ReqO or ReqO+data) if temporal locality is expected to be high, which can lead to improved cache efficiency, and reduced execution time and network traffic.
If stored data will not be accessed again by the writer, and/or the data is expected to be evicted before it is next accessed, 
write-through requests (ReqWT, ReqWT+data) may be used to avoid the indirection of remote ownership lookup.

\textbf{Dynamic granularity}: Requests may be issued at line granularity if spatial locality is expected to be high (improving cache efficiency, performance, and network traffic), or word granularity if spatial locality is expected to be low (reducing overheads of wasteful data movement).


\textbf{Write-through forwarding} changes how the Spandex LLC handles a write-through request for remotely owned data.
Rather than writing the specified data to the LLC, updating the LLC state to Valid, and forwarding an ownership request to the current owner, 
the write-through request is forwarded to the current owner without updating any state at the LLC.
This is similar to how a self-invalidated read (ReqV) request is handled, since neither a write-through request nor a ReqV updates state at the LLC.
As a result, a forwarded write-through request can similarly fail if ownership changes before the request arrives at the owner.
When this happens, the failed request must be Nacked and retried.
In addition, after some finite number of failures, a requestor must retry with a non-forwarded write-through request to prevent starvation in the presence of frequent ownership changes.

Write-through forwarding can be useful when write locality is low and the next consumer of written data is expected to currently own it.
From a programmer's perspective, a consumer may request ownership for some data in a buffer as a kind of pre-loading step, or if a space is repeatedly used for message passing the consumer can obtain ownership once on-demand and hit locally for subsequent accesses. %, or for the first load to a shared address space that is iteratively used for message passing.
Subsequently, the producer may use forwarded write-through requests to send the data directly to the consumer's cache, enabling it to hit on subsequent read accesses.
Since read latency is typically more important to performance than write latency, moving the overhead of data movement to the producer side is often beneficial.

\textbf{Owner prediction} takes advantage of Spandex support for self-invalidated reads and forwarded write-through requests to allow a device to predict the current owner of target data and send a request directly to that core.
This is identical to the direct cache-to-cache transfer optimization described by Choi et al. for self-invalidated reads in the original DeNovo protocol~\cite{ChoiKomuravelli2011}, 
but with Spandex it can be applied to write-through requests as well.
Neither request type affects state at the LLC; when the target data is remotely owned, the request is simply forwarded to the current owner.
This means that sending such a request directly to the current owner is functionally equivalent to looking up the current owner at the LLC.
In addition, since these forwarded messages are not serialized with other requests in Spandex (which may change the ownership state), and since Spandex assumes an unordered network,
the protocol must already account for forwarded ReqV or ReqWT requests arriving after ownership has been lost, prompting a retry.
Therefore, mispredicting an owner may have negative performance effects, but it will not break anything in the protocol.

If the current owner is known or can be predicted, using owner prediction to directly forward ReqV or ReqWT requests avoids the latency, traffic, and energy overheads of looking up the owner at the LLC.
If the physical location of the owner device can be predicted at compile time (e.g. there is a dataflow edge between fixed devices), this information may be included as a software hint.
Otherwise, a lightweight predictor could be used to guess the current owner based on past responses to forwarded ReqV or ReqWT requests.


Determining how best to use these specialized coherence request types is a significant challenge in itself, requiring knowledge about the memory demands of the workload.
%Efficiently mapping memory accesses to specialized Spandex request types requires some knowledge about the memory demands of the workload.
%Fortunately, 
Although outside the scope of this work, past research has focused on extracting this type of information statically from software, at compile time, or dynamically at runtime.
%The trend of increasing hardware specialization in many compute domains has been accompanied by an increase in specialized programming models,
%a wide range of specialized high level programming languages are simultaneously being developed to allow programmers to take full advantage of these new architectures.
%which are often domain-specific and can carry valuable information about memory access patterns.
For example, partitioned global address space (PGAS) programming models %allow the programmer to control the layout of data in a distributed memory system to improve locality and availability~\cite{YelickBonachea2007,ChamberlainCallahan2007,CharlesGrothoff2005,FatahalianHorn2006,}. 
%These programs therefore contain information about expected data access locality, visibility, and throughput demands.
carry explicit information about expected data access locality, visibility, and throughput demands that are used to guide the layout of data in a distributed memory system~\cite{YelickSemenzato1998,NumrichReid1998,CarlsonDraper1999,CharlesGrothoff2005,FatahalianHorn2006,YelickBonachea2007,ChamberlainCallahan2007,BauerTreichler2012},
scoped synchronization accesses in the HSA programming model carry information about synchronization locality~\cite{HSASpec},
\footnote{Although using the HRF memory model incurs undesirable complexity, we assume scopes may be used as optional hints to communicate expected locality in a DRF memory model.}
%in the HSA programming model adds significant complexity when paired with the HRF memory model, but if the simple DRF modle is used, scope semantics may still be used as a hint to communicate information about expected synchronization locality. %be used as hints about synchronization locality to improve memory system performance (e.g. as described in Section~\ref{sec:scopes-conc}).
and  dataflow programming languages offer explicit information about producer-consumer relationships and data movement granularity~\cite{ZahariaChowdhury2010,AbadiAgarwal2016}.
Sometimes locality and dataflow information is not statically available, or the optimal request types depend on the resources of the target system or how tasks are dynamically scheduled in a system. 
In these cases, request types may be selected based on compile-time analysis  %(e.g. ~\cite{WangMcKinley2002}) 
or runtime profiling. % (e.g. ~\cite{KooOh2017}).

\section{Complexity Analysis}
\label{sec:mem-opt-complexity}

Two of Spandex's biggest strengths are flexibility and simplicity: it offers a wide range of access types to fit any workload's memory demands while
avoiding much of the complexity that makes modern heterogeneous protocols so difficult to validate or extend.
The goals of flexibility and simplicity are often at odds with each other, and Spandex is able to achieve both by building upon the simple and efficient DeNovo protocol.
DeNovo relies on word granularity state and a DRF memory model to entirely avoid the need for transient blocking states.
Komuravelli and Adve used the Mur$\phi$ model checker tool~\cite{Dill1996} to compare the complexity of the DeNovo and MESI protocols and found MESI to be significantly more complex;
the Mur$\phi$ state space exploration %took 20x as long and 
explored 14x more states~\cite{KomuravelliAdve2015}.

Spandex extends DeNovo to support more request types, such as writer-invalidated reads and write-through stores and atomics.
This added flexibility introduces transient states and new race conditions, increasing the state space significantly.
However, since it is based on DeNovo rather than MESI, we claim it is still preferable to more conventional heterogeneous coherence solutions.

To evaluate this claim, we explore the DeNovo-based Spandex protocol state space in Mur$\phi$ and compare it against a MESI protocol (based on the implementation used by Multifacet GEMS~\cite{MartinSorin2005}) extended to implement a simplified version of non-snoopable request types similar to those of the ARM CHI~\cite{CHISpec}, described in Section~\ref{subsec:spandex-background-solns} \changes{with added support for accessing any data with any request type.}
%The detailed internal state transitions of ACE are not known; however, we implement non-cached loads and stores based on publicly available information on the ACE interface.
A flat cache organization was used instead of a hierarchical heterogeneous protocol such as that of the gem5 AMD APU~\cite{AMDgem5APU} because exhaustively exploring interactions between all devices in a multi-level protocol is expected to require a prohibitively large state space.
In addition, although Spandex supports variable request granularity, we do not explicitly model this in Mur$\phi$ and instead assume a fixed word granularity.
A Spandex system is expected to handle each word in a multi-word request individually based on its state. 
Therefore, we contend that adding support for coarse-grained or multi-word request types does not add any fundamental complexity to the protocol and would unfairly increase the state space in a Mur$\phi$ model.

Each of these protocols is then further extended with the write-through forwarding and owner prediction optimizations discussed in Section~\ref{sec:mem-opt-design}.
The actual CHI specification in fact supports a form of producer-consumer forwarding, referred to as cache stashing, and
cache stashing differs slightly from the optimizations described above (this difference is discussed in Section~\ref{sec:related} in more detail).
However, the above write-through forwarding and owner prediction optimizations are applied identically to both designs to ensure a fair comparison.

\begin{figure}[tb!]
%\begin{figure}[tbhp]
  \centering
%\begin{figure}[tb!]
  \includegraphics[width=\textwidth]{figures/complexity}
  \vspace{-3.5ex}
  \caption{State space comparison between Spandex and ARM CHI with added optimizations, writethrough forwarding (WTfwd) and owner prediction (Opred).}
  \label{fig:mem-opt-complexity}
  \vspace{-3ex}
%\end{figure}
\end{figure}

Figure~\ref{fig:mem-opt-complexity} plots the number of states explored by Mur$\phi$ for each protocol model.
Interestingly, the baseline Spandex protocol actually has slightly more states than the ARM CHI model.
This can be attributed to the fact that Spandex offers fundamentally more flexibility. 
\changesb{Rather than simply two types of loads and store requests (snoopable and non-snoopable), Spandex allows the programmer to specify whether or not a store requires up-to-date data as well, and thus requires considering two more L1-initiated request types that may be pending at the L1 or L2 at any time.}
This added flexibility allows a device to avoid much of the false sharing and transient states that are unavoidable in CHI, giving the developer some control over the magnitude of complexity-related overheads in a Spandex system.

As optimizations are added, the fundamental complexity of the MESI-based \changes{CHI} coherence solution becomes more evident.
Mur$\phi$ explores 1.1x more states in ARM \changes{CHI} with write-through forwarding (WTfwd) added to both protocols, and 2.1x more states with owner prediction (Opred) added.
This additional complexity can be explained by the fact that \changes{CHI} is based on a line-granularity read-for-ownership protocol, and this prioritization is reflected in the state transitions.
Every cache miss causes a transition to a transient state that blocks subsequent requests until some satisfying set of messages is received to transition back to a stable state.
In contrast, Spandex builds upon DeNovo (which has no transient states) and avoids blocking states as much as possible (they are only needed for transitioning to and from Shared state at the LLC, and for supporting ReqWT+data requests).
Spandex therefore avoids much of the state space explosion that can occur when adding optimizations to a protocol with excessive transient states. In fact, there is little increase at all in the number of Spandex states.





\section{Evaluation}
\label{sec:mem-opt-evaluation}

\subsection{Methodology}
\label{subsec:mem-opt-methodology}
To evaluate the above dynamic coherence flexibility, we use an integrated CPU-GPU architectural simulator with six architectural configurations.
The simulator is identical to the simulator used in Section~\ref{sec:spandex-results} with added support for dynamic request selection and write-through forwarding.
The first four configurations (SMG, SMD, SDG, SDD) are the same as the Spandex configurations in Chapter~\ref{sec:spandex-results}.
Optimized Spandex (SO) uses selective dynamic request selection and (if beneficial) write-through forwarding to optimize memory system performance.
For this evaluation, the optimal memory request type is manually selected based on the known or profiled properties of the workload.
SO+pred adds owner prediction to SO, which means ReqV and ReqWT requests are sent directly to the current owner (modeled as an oracle prediction, using the current state at the LLC).

We compare these configurations using a set of synthetic microbenchmarks %and real applications.
%The microbenchmarks 
which highlight the value of these memory optimizations.
%These include the microbenchmarks studied in Chapter~\ref{chap:spandex} as well as additional benchmarks which highlight the value of memory performance extensions.
These benchmarks and the manually chosen request types for each are described next.

\begin{itemize}

\item \textbf{FlexV/S}: Highlights the benefits of dynamically choosing between writer-invalidated and self-invalidated reads.
CPU and GPU cores repeatedly access tiles in multiple arrays, and only some accesses exhibit inter-kernel reuse.
The CPU densely reads one array with high inter-kernel reuse (array A) and with overlap with other CPUs, then densely reads a second array with no inter-kernel reuse (array B).
The GPU sparsely stores to array A with no inter-kernel reuse, and densely reads and writes array B with high inter-kernel reuse.
In optimized Spandex, CPU loads to array A use writer-invalidated reads, while CPU loads to array B use self-invalidated reads.
GPU updates to array A use write-through requests, while GPU updates to array B obtain ownership.


\item \textbf{FlexO/WT}: This microbenchmark highlights the benefits of dynamically choosing between ownership-based stores and write-through stores.
It is similar to the ReqO microbenchmark from Section~\ref{sec:spandex-results} where CPU and GPU cores
take turns densely reading and writing one matrix with high inter-kernel reuse and sparsely reading a second matrix with low inter-kernel reuse.
However, in FlexO/WT the sparsely accessed matrix is written instead of read.
This sparse update exhibits low inter-kernel locality, so obtaining ownership is wasteful.
Optimized Spandex uses line granularity ownership requests for the dense writes with high locality and uses word granularity forwarded write-through requests for the sparse updates with low locality.

\item \textbf{FlexOd/WTd}: This microbenchmark highlights the benefits of dynamically choosing between ownership-based atomic accesses and write-through atomic accesses, as well as dynamic granularity selection.
Each core (CPU and GPU) atomically updates one matrix densely with high reuse potential and one matrix sparsely with low reuse potential (and in a racy manner).
The densely accessed matrix is also accessed sparsely by a remote core concurrently (motivating the atomic request type).
Optimized Spandex uses line-granularity ownership requests (ReqO+data) for atomic accesses with high reuse potential and uses word-granularity write-through requests (ReqWT+data) for atomic accesses with low reuse potential.

\item \textbf{Indirection}: This is the same as microbenchmark in Section~\ref{sec:spandex-results}, where CPU and GPU cores take turns reading a tile from one matrix and writing it to the transposed tile in another matrix.
Optimized Spandex obtains ownership for reads and uses forwarded write-through requests for the writes.
%This optimization moves the overhead of data movement from the reader side to the writer side and avoids the overheads of owner lookup at the LLC.
\end{itemize}


\subsection{Results}
\label{subsec:mem-opt-results}

\begin{figure}[tb!]
%\begin{figure}[tbhp]
  \centering
  %\subfloat[Execution time]{
  \begin{subfigure}[b]{0.95\textwidth}
    %\includegraphics[scale=0.33]{figures/spandex/ubmk-cycles}
    \includegraphics[width=\textwidth]{figures/mem_opt/ubmks-cycles}
    \label{fig:mpe-ubmks-cycles}
    \caption{Execution time}
  \end{subfigure}
    \begin{subfigure}[b]{0.95\textwidth}
    \includegraphics[width=\textwidth]{figures/mem_opt/ubmks-nw}
    \label{fig:mpe-ubmks-nw}
    \caption{Network traffic}
  \end{subfigure}
%  \vspace{-2ex}
  %\subfloat[Network Traffic]{
  %  %\includegraphics[scale=0.33]{figures/spandex/ubmk-nw}
  %  \includegraphics[width=0.47\textwidth]{figures/spandex/ubmk-nw}
  %  \label{fig:ubmks-nw}
  %}
%  \vspace{-2ex}
  \caption{Synthetic microbenchmarks execution time and network traffic, normalized to SMG.}
 \label{fig:mpe-ubmks}
  \vspace{-2ex}
\end{figure}

Figure~\ref{fig:mpe-ubmks} shows the execution time and network traffic for the microbenchmarks.
Network traffic is broken down by request type as in Sections~\ref{subsec:scopes-denovo-eval} and \ref{sec:spandex-results}. 
Sbest represents the best performing (lowest execution time) non-optimized Spandex configurations for each microbenchmark averaged over all microbenchmarks.

For \textbf{FlexV/S}, the best performing non-optimized configurations are SMG and SMD, so the use of writer-invalidated reads at the CPU is clearly important to performance.
Obtaining Shared state for the dense read accesses with inter-kernel reuse improves CPU cache hit rates, reducing latency and traffic for these CPU read accesses.
Obtaining Shared state for the sparse read accesses with no inter-kernel reuse is wasteful, and requires revoking ownership (when enabled) from a remote GPU core. Revoking this ownership also prevents inter-kernel reuse at the GPU.
Optimized Spandex requests line granularity Shared state for the dense reads with inter-kernel reuse and it uses word granularity self-invalidated reads for the sparse accesses with no reuse.
It therefore offers high cache hit rates for the data with high locality while avoiding the overheads of Shared state where it is wasteful (and allowing the GPU to exploit reuse in owned data). 
SO as a result reduces network traffic by 50\% relative to the fastest non-optimized configuration, SMG (42\% relative to the configuration with lowest network traffic, SMD).
However, performance is dominated by the latency of the CPU accesses, which exhibit high potential for reuse, and SO's ability to avoid wasteful shared state and improve GPU reuse only decreases total execution time by 3\% relative to SMG (GPU performance is less sensitive to memory latency).
With ownership prediction (SO+pred), avoiding the indirection of lookups at the LLC for ReqV and ReqWT requests does not significantly improve performance,
reducing network traffic only by an additional 5\% and execution time an additional 2\% relative to SO.
%\marks{
This is because forwarded ReqV requests do not carry data, so they do not contribute significantly to total traffic. In addition, owner prediction can only change a three-hop miss to a two-hop miss. This latency difference is relatively small, and it only affects a subset of CPU accesses, reducing the impact of the optimization.
%}


For \textbf{FlexO/WT}, execution time is relatively constant among non-optimized configurations, but network traffic varies greatly. 
This workload exhibits significant inter-kernel reuse in written data, so obtaining ownership for writes is important.
Since overall performance is most sensitive to CPU memory latency and all configurations obtain ownership for writes at the CPU, there is not much difference in execution time.
On the GPU, however, only SMD and SDD obtain ownership for writes, and the improved GPU cache hit rate reduces network traffic by up to 65\% among non-optimized Spandex configurations (SDD vs. SDG).
FlexO/WT also contains sparse stores to remotely owned data, which exhibit no inter-kernel reuse and require revoking ownership from the core that experiences reuse in unoptimized Spandex.
Optimized Spandex uses forwarded write-through requests for these stores, performing the updates in place at the current owner and avoiding a wasteful ownership revoke. % for data which exhibits reuse at the remote owner.
As a result, Spandex increases the load hit rate for both CPU and GPU caches, reducing execution time by 19\% relative to the fastest non-optimized configuration (SMG) and network traffic by 87\% relative to the non-optimized configuration with the lowest network traffic (SDD).
With oracle ownership prediction, it is possible to reduce network traffic by an additional 34\% relative to SO.

For \textbf{FlexOd/WTd}, execution time and network traffic for non-optimized Spandex configurations are relatively constant apart from two outliers: exceptionally high execution time for SDG, and exceptionally low network traffic for SDD.
These differences are due to differences in the type of access used for atomics.
At the CPU, both DeNovo and MESI use ownership for atomics, but DeNovo uses word granularity while MESI uses line granularity.
Both are able to exploit reuse in the dense accesses with high inter-kernel locality, but for sparse accesses with no locality, MESI incurs overheads of false sharing by requesting ownership at line granularity.
This is seen in the high network traffic for SMG and SMD.
Interestingly, this false sharing overhead is also present in SDG. The reason for this has to do with how Spandex handles ReqWT+data requests for remotely owned data.
When a ReqWT+data request from the GPU arrives for data owned at the CPU, ownership is revoked at line granularity (this is done for simplicity and is not required for functionality).
In a MESI CPU, the first atomic access to the line in the subsequent iteration will retrieve ownership for the full line, exploiting spatial locality in dense atomic accesses.
However, DeNovo will request ownership for each word individually. This is what contributes to the significant performance degradation for SDG.
In contrast, with word granularity ownership requests at both the CPU and GPU, SDD is able to exploit reuse while avoiding the network traffic overheads of false sharing.
Optimized Spandex is able to treat atomic accesses individually: it uses word granularity write-through requests for sparse accesses with low locality, and line-granularity ownership requests for dense accesses with high locality.
For the sparse racy accesses to remote arrays, optimized Spandex uses word granularity ReqO+data to avoid revoking ownership at line granularity (as happens with SDG).
SO therefore exploits cache reuse where possible and avoids wasteful data movement when locality is not present.
It is able to reduce execution time even more than the fastest unoptimized configuration (6\% reduction relative to SMG),
and reduce network traffice even more than the unoptimized configuration with the least traffic (27\% reduction relative to SDD).
Owner prediction provides no benefit here since only atomic requests are used (only ReqV and ReqWT requests can be directly forwarded).

In \textbf{Indirection}, execution time is most affected by the choice of GPU protocol, while network traffic is most affected by the choice of CPU protocol.
Using DeNovo rather than GPU coherence at the GPU increases execution time because CPU cores read data written at the GPU.
Although obtaining ownership for writes at the GPU can reduce network traffic by avoiding data copies through the LLC, it adds indirection latency for reads at the CPU, increasing overall execution time.
Using MESI at the CPU can increase network traffic primarily due to false sharing.
In this tiled matrix transpose workload, loads exhibit high spatial locality, but multiple cores may store to a single cache line.
Using line-granularity ownership requests requires ownership transfer and data movement even when stores are to disparate words.
Optimized spandex avoids all of these overheads and is actually able to exploit reuse in reads despite the fact that read values are updated remotely between each kernel invocation.
It does this by obtaining ownership for loads, using write-through requests for stores, and using ownership prediction to send stores directly to the current owner.
%~\footnote{Currently oracle prediction is modeled, and the L2 cache state is queried to determine the predicted owner.}
By moving the overhead of data movement from the reader to the writer side, SO improves read hit rates, reducing
execution time by 33\% relative to the fastest non-optimized configuration (SDG).
However, indirection also highlights one side effect of write-through forwarding: forwarded write-through requests incur additional traffic. 
\marks{This is because update data must travel two hops: first to the LLC and then to the owning core. 
In contrast, configurations that obtain ownership for updates only need to transfer data one hop: from the owner to the requestor (all other hops do not transfer data).}
As a result, SO increases network traffic by 35\% relative to SDD (the unoptimized configuration with the lowest traffic).
However, this overhead can be avoided using ownership prediction, and SO+pred reduces network traffic by 54\% relative to SDD.

Overall, the flexibility offered by dynamic request selection, write-through forwarding, and owner prediction enables notable performance gains for the workloads studied.
SO (SO+pred) reduce execution time by on average 15\% (16\%) and network traffic by on average 55\% (63\%) relative to the fastest non-optimized Spandex configuration for the microbenchmarks studied.
Although not explored here, we intend to investigate the benefits of dynamic coherence specialization in real heterogeneous applications in future work.

%applications
%\begin{itemize}
%\item  bc with line ownership?
%\item  pagerank cpu with shared state?
%\item  rsct with forwarded atomics
%\item  hsti/o with line ownership?
%\item  tqh with WT atomics?
%\end{itemize}


\section{Summary}
\label{sec:mem-opt-summary}

As computer systems become more parallel and heterogeneous, flexible memory systems like Spandex are needed to support their increasingly diverse memory demands.
The flexibility and simplicity of Spandex allow devices to dynamically adapt their coherence strategies to exploit predicted or statically known workload properties.
Spandex offers request type flexibility in the fundamental coherence dimensions of stale data invalidation, write propagation, and request granularity.
It is based on the simple DeNovo protocol, and this allows it to incorporate extensions and optimizations more easily than more complex MESI-based heterogeneous coherence solutions.

In this work we describe dynamic coherence specialization, additions to the memory request interface that enable software or a hardware predictor to tailor a coherence request type to the access properties of the executing workload.
While this additional information does not affect the functional semantics of memory accesses, we show that it can be used to improve memory system performance for a range of access patterns.
In addition, using the Mur$\phi$ model checker tool, we show that although baseline Spandex is slightly more complex than a conventional MESI-based heterogeneous protocol,
it is more flexible and easier to extend with optimizations.
Going forward, it will be important to examine the memory demands of future workloads to determine which types of coherence optimizations can offer the greatest benefits.




==> metho-nn.tex <==
\subsection{Neural Networks}
\label{subsec:methodology-nn}

A small set of machine-learning algorithms especially Convolutional Neural Networks~\cite{LecunBottou1998} and
Deep Neural Networks~\cite{HintonSrivastava2012}
%are proving to be state-of-the-art across many applications. % and 
are %simultaneously  
becoming pervasive in a broad range of systems from embedded systems to data centers. 
Currently, these neural networks are mostly executed on GPUs~\cite{CoatesHuval2013} to efficiently exploit the vast amount of parallelism available for computation of primitives. 

\textbf{Parallel NN} represents
the contemporary popular method of implementing neural networks on GPUs. It is essentially composed of a series of fully connected layers and parallelizes the input features across the compute units available on the GPU. As such, each compute unit executes its partitioned data in parallel through all the layers of the network.

On the other hand, an unconventional yet possible way of implementing a neural network is to distribute the layers of the network across the compute units of the GPU. Since the weights of a neural network exhibit the most reuse in many cases, allowing each layer to be computed in the same location each iteration enables the possibility of exploiting this temporal locality.

\textbf{Pipelined NN} represents
this method of implementing neural networks on GPUs. It distributes the series of fully connected layers to separate compute units and as a result, each layer is computed in the same location. The intermediate neuron values are transferred between the adjacent compute units using a producer-consumer message buffer pattern, and adjacent workers perform fine-grained synchronizations to let the consumer know when the output is ready and to let the producer know when the buffer is safe to write to.


%An unconventional way of implementing a neural network is pipelining the layers to different cores on the GPU. Traditionally, pipelining a neural network layers has been dis-regarded because its implementation inevitably requires the addition of expensive overheads that did not exist in a more conventional data parallel implementaion. The atomic communications necessary between adjacent workers is one such overhead.  Furthermore, pipelining different layers to different cores introduces data races for the intermediate layer input/outputs that did not exist in a more conventional data-parallel counterpart. To make matters worse, since data races must be protected by synchronizations, its implementation required frequent yet expensive invalidations of the GPU’s L1 cache using traditional GPU coherencd protocol. ile this implementation essentially adds dependencies to the network that didnot exist to an original fully connected network, it allows the flexibility of Spandex and additional optimizations to show off its benefits

==> related_thesis.tex <==
\chapter{Related Work}
\label{chap:related}

\section{Performance Evaluation for High-Throughput Accelerators}
\label{sec:related-gsi}

There have been previous efforts to provide more detailed performance profiling
metrics for high-throughput accelerators such as GPUs.
GPGPU-Sim is a cycle-accurate GPU simulator that can be used to model the 
effects of architectural changes to a GPU device~\cite{BakhodaYuan2009}.  It provides 
many simulation evaluation metrics including overall performance and stall 
counts, but not a stall breakdown.  Aerialvision~\cite{ArielFung2010} augments 
GPGPU-Sim to provide more detailed measurements such as the number of cycles 
spent in the core pipeline by each thread, the number of DRAM accesses 
generated by each instruction, and the number of stall cycles due to 
long-latency off-chip read requests. However, it lacks a single comprehensive 
breakdown attributing execution latency to fine-grained stall causes.

O'Neil and Burtscher~\cite{OneilBurtscher2014} use a stall classification method, also based 
on GPGPU-Sim, to help understand the performance of irregular GPU kernels.  
Their breakdown, however, does not differentiate between stalls due to memory 
or compute delays.  Lee and Wu~\cite{LeeWu2014} also use a similar GPU stall 
classification method based on GPGPU-Sim which is designed to characterize the 
latency-hiding capability of GPU warp schedulers.  It provides a more detailed 
stall breakdown and adds a memory latency stall type, but is focused on 
warp scheduler changes.
% MDS (10/9/15): Too informal
%% and so is not very informative when it comes to stalls that are caused by memory latency.  

While this prior work also provides profiling information about GPUs, 
unlike GSI, they are all designed for discrete GPUs.  Furthermore, they 
focus on profiling the GPU core, while we are capturing detailed information 
about the causes of memory stalls in a unified CPU-GPU memory system.

\section{Efficient Heterogeneous Coherence and Coherence Integration}
\label{sec:related-hetero-coh-int}

Many prior innovations aim to both improve heterogeneous coherence and integrate heterogeneous caches. We therefore discuss work related to the contributions in Chapters~\ref{chap:scopes} and \ref{chap:spandex} together.
We omit discussion of HRF and RSP, which are described in Section~\ref{sec:scopes-background}, as well as IBM CAPI, AMD APU, and ARM CHI, which are described in Section~\ref{sec:spandex-background}.

\mmarks{There are multiple ongoing industry efforts to define communication interfaces between devices in heterogeneous systems.
For example, CCIX~\cite{CCIXSpec}, Gen-Z~\cite{GenZSpec}, and OpenCAPI~\cite{OpenCAPISpec} present interfaces for performing cached or non-cached coherent read and write accesses in a heterogeneous system.
These interfaces are more expressive than Spandex in some respects. For example, by offering an interface for attached devices to act as the home memory node for an address range or by offering bulk cooperative synchronization transactions such as reduce and gather/scatter operations.
They also offer more low-level flexibility regarding routing, packet loss and error correction/detection, and general physical layer configuration options.
However, at the time of writing, the underlying coherence protocol and state transition internals at the host/responder/home agent (in OpenCAPI/Gen-Z/CCIX terminology, respectively) for these interfaces are not publicly available.
%However, at the time of writing, these specifications are either not publicly available (e.g., CCIX~\cite{CCIXSpec}, Gen-Z~\cite{GenZSpec}) or do not implement coherent caching for accelerators (e.g., OpenCAPI~\cite{OpenCAPISpec}).
Marvell MoChi is a modular chiplet architecture that promises seamless integration between components~\cite{MoChiSpec}, but again, a detailed specification of any coherence interface between these chips is not publicly available.
The fact that there are so many active industry efforts to address this challenge serves to reinforce its growing importance.
Though many implementation details are still not public or are under development for these integration strategies, the insights presented in this work may serve to motivate a focus on simplicity and flexibility in future iterations.}
%The Gen-Z~\cite{GenZSpec} and OpenCAPI~\cite{OpenCAPISpec} interfaces do not currently implement full coherence between accelerator devices.
%CCIX~\cite{CCIXSpec} promises coherence, however this specification is not yet publicly available.
%\footnote{ARM CCI CoreLink Cache Coherent Interconnect implements ACE-Lite using a centralized snoop filter to improve scalability, but }


%In addition to the existing hardware mechanisms discussed in Section~\ref{subsec:background-solns}, 
Past work has implemented efficient CPU-GPU coherence, using both hardware and software techniques.
QuickRelease (QR)~\cite{HechtmanChe2014}, Heterogeneous System Coherence (HSC)~\cite{PowerBasu2013}, and the Fusion architecture~\cite{KumarShriraman2016} all use a clustered hierarchical cache structure and MESI-based last level directory to interface CPU and GPU devices. 
Software-managed page migration strategies that intelligently perform explicit page copies between CPU and GPU memories 
have also been shown to be effective for many CPU-GPU workloads~\cite{NegrutSerban2014,Sakharnykh2016,AgarwalNellans2016}.
%QR implements non-blocking stores using a hierarchical S-FIFO which can coalesce writes and reduce invalidation probes when spatial locality is high, and HSC uses coarse-grain region coherence at the directory, which can similarly reduce probe messages when spatial locality is high. 
However, all of these techniques rely on dense, hierarchical sharing patterns to be effective,
and performance can suffer for new or irregular sharing patterns due to the high cost of inter-device communication.

Interfacing heterogeneous protocols can be avoided by using the same protocol at both CPU and GPU L1 caches. Temporal coherence~\cite{SinghShriraman2013}, VIPs-G~\cite{KoukosRos2016}, and even DeNovo for GPUs~\cite{SinclairAlsop2015} adopt this approach. However, the design of an L1 interface is often tightly integrated with processor design, and 
%redesigning all cores to interface with a new cache protocol may be an unacceptable design burden.
requiring all cores to interface with a new cache protocol may be an unacceptable design burden. 
%In contrast, Spandex offers a solution that can interface a wider range of CPU and GPU protocols, enabling the use of existing IP without significant design changes, and enabling more flexibility in the design of future specialized caches.


%There have been many recent efforts in industry and academia to improve coherence support for emerging heterogeneous devices.

%Hechtmann and Sorin proposed a flat MOESI-based coherence strategy for tighly coupled CPU-GPU systems which implements an SC consistency model~\cite{HechtmanSorin2013,HechtmanSorin2013_2}. However, they do not evaluate the overheads of MOESI or compare against other coherence strategies.


%%The IBM Coherent Accelerator Processor Interface (CAPI) enables FPGA and other accelerators to use a coherent MESI-based cache which interfaces with a snoopy MESI-based last level cache fabric~\cite{StuecheliBlaner2015}. 
%The IBM Coherent Accelerator Processor Interface (CAPI) enables FPGA and other accelerators to interface with %use a coherent MESI-based cache which interfaces with 
%a snoopy MESI-based last level cache fabric~\cite{StuecheliBlaner2015}. 
%%This design enables efficient high-bandwidth communication between accelerators which share a cache or between CPUs in a cluster, but 
%Here the use of a MESI-based protocol means that memory demands which are unsuitable for MESI can suffer from excessive coherence overheads.
%Similarly, the AMD APU simulator architecture uses a hierarchical cache structure with a MESI-based directory/probe filter to interface CPU and GPU core clusters~\cite{BeckmannGutierrez2015}. This hierarchical structure means communication between CPU and GPU cores suffers added latency and energy overhead due to indirection through hierarchical cache layers.


%ARM has introduced AXI Coherence Extensions (ACE and ACE-lite), two open specifications for a bus-based coherence interface which can be used for accelerators~\cite{ACESpec}. 
%ACE allows an accelerator cache to use a MOESI protocol, with shared and modified state requested and revoked via a snoop channel. ACE-lite allows an accelerator cache to use a simpler protocol similar to GPU coherence, which uses self-invalidation and a write-through cache rather than snoop requests to keep data coherent. 
%These two coherence options offer improved flexibility with respect to other existing heterogeneous coherence strategies, 
%The ARM ACE-lite coherence interface allows an accelerator to use a simpler protocol which is similar to GPU coherence, with "uncached" read and write requests of varying granularity. 
%However, the coherence implementation is not publicly available.
%the use of a snoop-based MOESI last level interface and the fixed granularity state limit protocol scalability and flexibility.


%The challenge of interfacing heterogeneous protocols can be avoided by using the same protocol at both CPU and GPU L1 caches. This is the strategy taken by both DeNovo for GPUs~\cite{SinclairAlsop2015} and VIPs-G~\cite{KoukosRos2016}. However, the design of an L1 interface is often tightly integrated with processor design, and 
%%redesigning all cores to interface with a new cache protocol may be an unacceptable design burden.
%requiring all cores to interface with a new cache protocol may be an unacceptable design burden. 
%%In contrast, Spandex offers a solution that can interface a wider range of CPU and GPU protocols, enabling the use of existing IP without significant design changes, and enabling more flexibility in the design of future specialized caches.

%In the realm of multicore CPU coherence, t

Crossing Guard offers a simple and stable coherence interface for accelerator caches~\cite{OlsonHill2017}. However, Crossing Guard's primary goal is correctness and security in heterogeneous coherence, not improved performance. It also only interfaces with MESI and MOESI style caches. Thus it is unclear whether accelerator caches that prefer simpler protocols such as GPU coherence or DeNovo would be able to efficiently interface with the system.

Manager-client pairing (MCP) is a framework for defining hierarchical coherence protocols in large-scale systems~\cite{BeuRosier2011}. Like Spandex, MCP addresses the complexity of hierarchical protocols and evaluates the costs of deeper cache organizations. However, MCP is focused on providing a generic framework for building hierarchical protocols for devices that request read and write permission.
Spandex instead aims to avoid the need for hierarchical organization for a wide variety of heterogeneous devices, some of which use self-invalidations or write-through caches instead of requesting read/write permissions, and which can use variable request granularity.


%NVIDIA, AMD, IBM, and ARM have all proposed some form of heterogeneous coherence.
%Unified memory, introduced in CUDA 6, enables transparent sharing between CPU and GPU devices through automatic runtime-managed page migration~\cite{NegrutSerban2014,Sakharnykh2016}. 
%Agarwal et al. use a similar mechanism to show that a carefully designed software-managed caching strategy can approach hardware performance for many common GPU application access patterns~\cite{AgarwalNellans2016}.
%However, runtime-managed coherence can suffer when faced with new or irregular sharing patterns due to the high potential cost of a miss.

%\hilight{
Past work has also addressed the challenge of enforcing memory consistency in heterogeneous systems. ArMOR provides a framework for precisely defining the ordering requirements of different consistency models and 
%introduces the notion of translator shims, which ensure 
ensures that 
devices with different memory models respect ordering constraints in a heterogeneous system~\cite{LustigTrippel2016}.
The Princeton Check family of tools offer a framework for specifying and verifying memory consistency ordering constraints, considering microarchitectural through application level concerns in the design of a coherent device~\cite{TrippelManerkar2017,ManerkarLustig2017,LustigTrippel2016,LustigSethi2016,ManerkarLustig2015,LustigPellauer2014}.
These techniques may be used in conjunction with Spandex when designing and integrating new device types. % in a heterogeneous system.

\section{Atomic Relaxation in Heterogeneous Systems}
\label{sec:related-relaxed}

%TODO: discuss outlawing ghosts, brian demsky checking concurrent data structures in c11,
%mathematizing c++, overhauling SC atomics: axiomatic definitions of mem model, don't address OOTA
%outlawing ghosts, OOTA{BoehmDemsky2014,BattyMemarian}: describes OOTA and dangers, to prevent OOTA results, enforce LD->ST reordering
%checking concurrent data structures{NorriSDemsky2013}:
%promising semantics{KangHur2017}:
%concurrency semantics{Pichon-PharabodSewell2016}:



Many existing memory models attempt to formalize allowed behavior in the presence of relaxed atomics while also prohibiting the strange behavior that can arise from out-of-thin-air (OOTA).
Boehm and Demsky thoroughly describe the problem of OOTA and propose a solution - preserving load-store ordering - which would prohibit common existing performance optimizations which exist in current hardware~\cite{BoehmDemsky2014}.
%Existing memory models deal with this problem in different ways.
The HSA memory model conservatively prohibits dependency cycles, preventing some desirable optimizations~\cite{HSASpec}.
The Java memory model~\cite{MansonPugh2005} defines complex semantics which aim to enable as many optimizations as possible, but has been found to unintentionally restrict some very common ones~\cite{VsevvcikAspinall2008}, and no fix has yet been proposed.
The C++11 memory model also was found to unintentionally restrict certain executions~\cite{BoehmAdve2008, Boehm2013}, and C++14 simply informally states that systems should not produce out-of-thin-air values~\cite{Boehm2013-2}.

Other attempts at formalization rely on difficult to understand concepts such as event structures and promise semantics~\cite{Pichon-PharabodSewell2016, KangHur2017}.
In summary, existing solutions to the challenge of relaxed atomics are either too ambiguous or too complex, and none preserve the SC-centric semantics used by DRFrlx.

%\section{Coherence Integration in Heterogeneous Systems}
%\label{sec:related-int}

\section{Dynamic Coherence Specialization}
\label{sec:related-mem-opt}

%A large body of prior work aims to improve memory system performance 
%Many specialized programming models and runtime systems have been developed in recent years which aim to optimize memory performance in parallel systems.
%They do this either by optimizing data placement and task scheduling, 



\dmarks{Adaptive coherence strategies have been explored extensively in prior work to improve memory system performance.
Dynamic self invalidation (DSI) offers adaptivity in the form of tear-off blocks, which use self-invalidation to avoid the need for tracking sharers or sending invalidations for read data, effectively enabling dynamic selection of self-invalidated or writer-invalidated reads~\cite{LebeckWood1995}.
Last-touch prediction can be used to avoid the indirection of a remote read request for modified data by selectively writing back modified data to the directory when an instruction is expected to be the ``last touch" to that data~\cite{LaiFalsafi2000}.
It can achieve benefits similar to those obtained by dynamically selecting write-through or ownership-based stores.
Past work has also studied the benefits of flexible state or coherence granularity~\cite{TorrellasLam1994,ZhaoShriraman2013,CantinSmith2006,RothmanSmith2000,KumarZhao2012,DavariRos2015}, which show that adapting communication and state tracking granularity to the spatial locality of a program can reduce false sharing and enable more efficient data tracking, lookup, and transfer.
Finally, protocol extensions have been proposed which detect and predict specific sharing patterns, optimizing requests to reduce wasteful traffic and latency for those patterns~\cite{StenstromBrorsson1993,CoxFowler1993,KoufatyChen1996,AndersonKarlin1996,AbdelshafiHall1997,MukherjeeHill1998,KaxirasGoodman1999,BilirDickson1999,MartinHarper2003,ChengCarter2007,SomogyiWenisch2009,KurianKhan2013}.
%\marks{
All of the above innovations demonstrate the benefits of dynamic adaptability, and in some cases offer even more flexible control over granularity or data movement than Spandex request types.
The methods for detecting and predicting sharing patterns will be increasingly relevant to specialized memory systems, and they could be used to help guide Spandex request type selection.
Even so, all of the above innovations focus on optimizing communication patterns in the context of MESI-based multicore CPU coherence.
As a result, their flexibility is limited, each focusing on adaptivity within a single coherence design dimension, and the benefits they provide often come at the cost of additional overhead and complexity on top of an already complex MESI-based protocol.
In contrast, Spandex is designed to offer comprehensive coherence flexibility while retaining a simple protocol with minimal coherence overheads.
}
%This protocol is similar to Spandex in that it offers the ability to dynamically trade off coherence complexity/overhead and cache efficiency. Unlike Spandex, DSI does not interface protocols like GPU coherence that use write-through caches and word-based request granularities.


Many studies also have proposed ways to improve memory access efficiency through adaptive cache management (replacement, prefetching, bypassing) in both CPUs and GPUs based on hints from the software, compiler, or runtime profilers~\cite{WangMcKinley2002,BeylsDhollander2005,YangGovindarajan2005,PapaefstathiouKatevenis2013,SethiaDasika2013,ChenChang2014,TianPuthoor2015,LiangXie2015,KooOh2017}.
These techniques allow caches to adapt to different access patterns and improve cache efficiency, and many of the insights regarding cache policy prediction can be leveraged to help select Spandex request types.
However, their flexibility is constrained to cache management policies rather than the fundamental coherence protocol flexibility offered by Spandex.

Expressive memory was recently proposed by Vijaykumar et al. as a framework for communicating high level properties of a program's memory access pattern to the underlying hardware to guide architectural optimizations, primarily in multicore CPUs~\cite{VijaykumarJain2018}. 
Similarly, the locality descriptor communicates high level information about data access locality in GPU programs to guide thread block scheduling and data placement in GPUs~\cite{VijaykumarEbrahimi2018}.
Both of these innovations exploit high level information from software to adaptively optimize memory system performance.
These techniques are entirely compatible with a Spandex system, and they could be used to take advantage of dynamic coherence specialization by guiding request type selection.

\changesb{
The ARM CHI interface supports a mechanism for producer-consumer forwarding called cache stashing.
This is similar to the write-through forwarding and owner prediction optimizations described in Chapter~\ref{chap:mem-opt} in that a producer device provides a hint to the system regarding the expected location of the consumer of some data.
However, unlike the write-through forwarding and owner prediction optimizations, cache stashing causes exclusive ownership to transfer to the target cache.
Although this avoids the need for the consumer to pre-emptively obtain ownership, it incurs additional complexity in the form of transient states,
and it prevents direct device-to-device communication since a stash request may change the owner state at the home node.
}



==> tables/dev_req_mapping.tex <==
\begin{table}
%\begin{center}
\centering
%\resizebox{0.5\textwidth}{!}{\begin{minipage}{\columnwidth}
\caption{Type and granularity of requests generated for read misses, write misses, and replacements of owned data in GPU coherence, DeNovo, and MESI caches. *A DeNovo ReqV request  is issued at word granularity, but the responding device may include any available up-to-date data in the line.}
\begin{tabular}{| c | c | c | c |} 
\hline
\textbf{\makecell{Device \\ Type}} & \textbf{\makecell{Device \\ Request}} & \textbf{\makecell{Spandex \\ Request}} & \textbf{Granularity} \\ \hline

\multirow{4}{*}{\makecell{GPU Coherence}} & Read & ReqV & line \\ \cline{2-4}
% * <sadve@illinois.edu> 2018-04-23T21:38:08.886Z:
% 
% Horizontal line missing between gpu and denovo
% 
% ^.
& Write & ReqWT & word \\ \cline{2-4}
& RMW & ReqWT+data & word \\ \hline %\cline{2-4}
% * <sadve@illinois.edu> 2018-04-21T18:29:04.687Z:
% 
% ReqRMW --> ReqWT+data??? Also is this word granularity? I think word for write, line for read? If so, needs to be said in a non-confusing way. I need to see it.
% 
% ^ <joalsop@gmail.com> 2018-04-24T00:37:53.468Z:
% 
% it's word
%
% ^.
%& Dirty Repl & ReqWT & word \\ \hline
% * <sadve@illinois.edu> 2018-04-21T18:30:40.972Z:
% 
% I don't understand DirtyRepl for GPU. There is no dirty state. And saying this is at word granularity is quite confusing to me.
% 
% ^ <joalsop@gmail.com> 2018-04-24T00:36:59.244Z.

\multirow{4}{*}{DeNovo} & Read & ReqV & flexible* \\ \cline{2-4}
% * <sadve@illinois.edu> 2018-04-21T18:32:03.872Z:
% 
% Above, what is meant by flexible needs explanation somewhere.
% 
% ^.
& Write & ReqO & word \\ \cline{2-4}
& RMW & ReqO+data & word \\ \cline{2-4}
% * <sadve@illinois.edu> 2018-04-21T18:33:57.176Z:
% 
% Isn't it line for read, word for write? Again, I'd like to see the outcome of this fix.
% 
% ^ <joalsop@gmail.com> 2018-04-21T22:03:48.009Z:
% 
% we call denovo read 'flexible' because it may respond with only the requested words, but it may also respond with other words in that line, depending on where the data is owned
%
% ^ <joalsop@gmail.com> 2018-04-24T00:36:48.949Z.
& Owned Repl & \makecell{ReqWB} & word \\ \hline

\multirow{4}{*}{MESI} & Read & ReqS & line \\ \cline{2-4}
& Write & ReqO+data & line \\ \cline{2-4}
& RMW & ReqO+data & line \\ \cline{2-4}
& Owned Repl & \makecell{ReqWB} & line \\ \hline
% * <sadve@illinois.edu> 2018-04-21T18:34:25.350Z:
% 
% Why is this word? Did we make this change to standard MESI? If so, we should say explicitly. If not, then fix.
% 
% ^ <joalsop@gmail.com> 2018-04-24T00:36:41.531Z.

\end{tabular}

\label{table:dev_req_mapping}
%\end{minipage}}
\end{table}


==> tables/spandex_reqold.tex <==
\begin{table}
%\begin{center}
\centering
{\footnotesize
%\resizebox{0.5\textwidth}{!}{\begin{minipage}{\columnwidth}
\begin{tabular}{| c | c | c | c | c |} 

\hline
\textbf{\makecell{Coherence \\ Dimension}} & \textbf{\makecell{Options}} & \textbf{\makecell{Request \\ Type}} & \textbf{\makecell{Sent to}} & \textbf{\makecell{Used For}} \\ \hline

\multirow{3}{*}{\makecell{Stale Data \\ Invalidation}} & \multirow{2}{*}{\makecell{Self-inval.}} & ReqV & LLC & \makecell{DeNovo (LD) \\ GPUc (LD) } \\ \cline{3-5}

 & & \textbf{ReqVo} & \textbf{\makecell{predicted \\ owner}} & \textbf{FCS(LD)} \\ \cline{2-5}

 & \makecell{Writer-inval.} & ReqS & LLC & \makecell{MESI (LD)} \\ %\cline{2-5}
 %& \makecell{Ownership} & ReqO+data & \makecell{--} \\ 
 \hline

 \multirow{5}{*}{\makecell{Update \\ Propagation}} & \multirow{2}{*}{Ownership} & ReqO & LLC & DeNovo (ST)\\ \cline{3-5}

 & & ReqO+data & LLC & \makecell{MESI (ST,RMW) \\ DeNovo (RMW) \\ \textbf{FCS(LD)}} \\ \cline{2-5}

 & \multirow{3}{*}{\makecell{Write- \\ through}} & ReqWT\textbf{[fwd]} & LLC & \makecell{GPUc (ST) \\ \textbf{FCS(ST)}} \\ \cline{3-5}

 & & \textbf{ReqWTo} & \textbf{\makecell{predicted \\ owner}} & \makecell{\textbf{FCS(RMW)}} \\ \cline{3-5}

 & & ReqWT\textbf{[fwd]}+data & LLC & \makecell{GPUc (RMW) \\ \textbf{FCS(RMW)}} \\ \cline{3-5}

 & & \textbf{ReqWTo+data} & \textbf{\makecell{predicted \\ owner}} & \textbf{\makecell{FCS (RMW)}} \\ \hline

\multirow{2}{*}{\makecell{Request \\ Granularity}} & Word & all & any & \makecell{DeNovo (all) \\ GPUc (ST,RMW)} \\ \cline{2-5}

 & Line & all & any & \makecell{MESI (all) \\ GPUc (LD)} \\ \hline

\end{tabular}
%\caption{\fontsize{9pt}{11pt}  Mapping of loads (LD), stores (ST) and atomics (RMW) in a DeNovo, GPU coherence (GPUc), or MESI protocol to Spandex request types.} 
\caption{Coherence request type classification and what they are used for in a DeNovo, GPU coherence (GPUc), or MESI protocol. Spandex is a coherence interface that can integrate devices that use any of these protocols. FCS adds flexibility by supporting fine-grain request selection and new coherence request types (in bold).} 

\label{table:spandex_reqs}
%\end{minipage}}
\vspace{-2ex}
}
\end{table}


==> use_case.tex <==
\section{}
